Generation-Augmented Retrieval for Open-domain Question Answering

We propose Generation-Augmented Retrieval (GAR) for answering open-domain questions, which augments a query through text generation of heuristically discovered relevant contexts without external resources as supervision. We demonstrate that the generated contexts substantially enrich the semantics of the queries and GAR with sparse representations (BM25) achieves comparable or better performance than state-of-the-art dense retrieval methods such as DPR. We show that generating diverse contexts for a query is beneficial as fusing their results consistently yields better retrieval accuracy. Moreover, as sparse and dense representations are often complementary, GAR can be easily combined with DPR to achieve even better performance. GAR achieves state-of-the-art performance on Natural Questions and TriviaQA datasets under the extractive QA setup when equipped with an extractive reader, and consistently outperforms other retrieval methods when the same generative reader is used.

==> Generation-Augmented Retrieval_arXiv/generation_eg.tex <==
\begin{table*}[ht]
        \resizebox{1.98\columnwidth}{!}{
        \begin{tabular}{p{17cm}}
            \toprule
            
            \textbf{Question}: when did bat out of hell get released?  \\
             \textbf{Answer}: \colorG{September 1977} \quad \colorB{\{September 1977\}} \\
             \textbf{Sentence}: Bat Out of Hell is the second studio album and the major - label debut by American rock singer Meat Loaf ... released in \colorG{September 1977} on Cleveland International / Epic Records.
             \\ \colorB{\{The album was released in September 1977 on Cleveland International / Epic Records.\}}\\
             \textbf{Title}: \colorG{Bat Out of Hell} \quad \colorB{\{Bat Out of Hell\}}\\
             
            \midrule
                \textbf{Question}: who sings does he love me with reba?  \\
             \textbf{Answer}: \colorR{Brooks \& Dunn}  \quad \colorB{\{Linda Davis\}} \\
             \textbf{Sentence}: \colorG{Linda Kaye Davis} ( born November 26, 1962 ) is an American country music singer. 
             \\ \colorB{\{`` Does He Love You '' is a song written by Sandy Knox and Billy Stritch, and recorded as a duet by American country music artists Reba McEntire and Linda Davis.\}} \\
             \textbf{Title}: \colorG{Does He Love Me} [SEP] \colorG{Does He Love Me (Reba McEntire song)} [SEP] I Do (Reba McEntire album) 
             \colorB{\{Linda Davis [SEP] Greatest Hits Volume Two (Reba McEntire album) [SEP] Does He Love You\}}\\
             
            \midrule
            \textbf{Question}: what is the name of wonder womans mother?  \\
             \textbf{Answer}: \colorR{Mother Magda} \quad\colorB{\{Queen Hippolyta\}} \\
             \textbf{Sentence}: In the Amazonian myths, she is the daughter of the Amazon queen Sifrat and the male dwarf Shuri, and is the mother of Wonder Woman. \quad\colorB{\{Wonder Woman's origin story relates that she was sculpted from clay by her mother Queen Hippolyta and given life by Aphrodite.\}}\\
             \textbf{Title}: \colorG{Wonder Woman} [SEP] \colorG{Diana Prince} [SEP] \colorG{Wonder Woman (2011 TV pilot)} 
             \\ \colorB{\{Wonder Woman [SEP] Orana (comics) [SEP] Wonder Woman (TV series)\}}\\
             

            \bottomrule
        \end{tabular}
        }
    \upv
    \caption{\textbf{Examples of generated query contexts}. \colorG{Relevant} and \colorR{irrelevant} contexts are shown in green and red. \colorB{Ground-truth references} are shown in the \{braces\}. The issue of generating wrong answers is alleviated by generating other contexts highly related to the question/answer.}
    \label{tab:generation_eg}
    \downv
    \end{table*}

==> Generation-Augmented Retrieval_arXiv/macro.tex <==
\usepackage{amsmath,amsfonts,bm}
\usepackage{booktabs} %
\usepackage{url}
\usepackage{graphicx}
\usepackage{array}
\usepackage{color}
\usepackage{makecell}
\usepackage{multirow}
\usepackage{xspace}

\newcommand{\yuning}[1]{\textcolor{cyan}{[Yuning: #1]}}
\newcommand{\xiang}[1]{\textcolor{red}{[Xiang: #1]}}
\newcommand{\qu}[1]{\textcolor{blue}{[kevin: #1]}}
\newcommand{\red}[1]{\textcolor{red}{#1}}
\newcommand{\cyan}[1]{\textcolor{cyan}{#1}}
\newcommand{\ie}{\textit{i.e.}} %
\newcommand{\eg}{\textit{e.g.}} %
\newcommand{\start}[1]{\vspace{.4mm}\noindent{{\bf #1}.}}
\DeclareMathOperator*{\argmin}{arg\,min\,}
\DeclareMathOperator*{\argmax}{arg\,max\,}
\newcommand\numberthis{\addtocounter{equation}{1}\tag{\theequation}}


\newcommand{\upv}{\vspace{-.0cm}}
\newcommand{\downv}{\vspace{-.1cm}}
\newcommand{\upvf}{\vspace{-.2cm}}
\newcommand{\downvf}{\vspace{-.2cm}}
\newcommand{\upve}{\vspace{-.0cm}}
\newcommand{\downve}{\vspace{-.0cm}}

\newcommand{\ours}{\textsc{Gar}\xspace}
\newcommand{\oursPlus}{$\textsc{Gar}^{\texttt{+}}$\xspace}

\definecolor{gred}{RGB}{219,68,55}
\definecolor{gblue}{RGB}{66,133,244}
\definecolor{gyellow}{RGB}{244,180,0}
\definecolor{ggreen}{RGB}{15,157,88}
\definecolor{ggrey}{RGB}{115,115,115}

\newcommand{\hlpgen}[2]{\fboxsep1pt \colorbox{ggreen!#2}{\strut #1}} %
\newcommand{\hlcov}[2]{\fboxsep1pt \colorbox{gyellow!#2}{\strut #1}} %
\newcommand{\colorR}[1]{\textcolor{gred}{\textbf{#1}}}
\newcommand{\colorG}[1]{\textcolor{ggreen}{\textbf{#1}}}
\newcommand{\colorB}[1]{\textcolor{gblue}{#1}}
\newcommand{\colorGrey}[1]{\textcolor{ggrey}{\textbf{#1}}}

